Controlling transient gas flow in real-world pipeline intersection areas

Compressor stations are the heart of every high-pressure gas transport network. Located at intersection areas of the network they are contained in huge complex plants, where they are in combination with valves and regulators responsible for routing and pushing the gas through the network. Due to their complexity and lack of data compressor stations are usually dealt with in the scientific literature in a highly simplified and idealized manner. As part of an ongoing project with one of Germany's largest Transmission System Operators to develop a decision support system for their dispatching center, we investigated how to automatize control of compressor stations. Each station has to be in a particular configuration, leading in combination with the other nearby elements to a discrete set of up to 2000 possible feasible operation modes in the intersection area. Since the desired performance of the station changes over time, the configuration of the station has to adapt. Our goal is to minimize the necessary changes in the overall operation modes and related elements over time, while fulfilling a preset performance envelope or demand scenario. This article describes the chosen model and the implemented mixed integer programming based algorithms to tackle this challenge. By presenting extensive computational results on real world data we demonstrate the performance of our approach.

==> commands.tex <==
\RequirePackage{xspace}
\RequirePackage{accents}

%%-------------------------------------------------------------
%% Abbreviations
%%-------------------------------------------------------------
\newcommand{\myie}{i.e.}
\newcommand{\myIe}{I.e.}
\newcommand{\myeg}{e.g.}
\newcommand{\myst}{s.t.\ }
\newcommand{\myWlog}{W.l.o.g.\ }
\newcommand{\mywlog}{w.l.o.g.\ }
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% nice underbar, needs 'accents' package
%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\ubar}[1]{\underaccent{\bar}{{#1}}}

\newcommand{\ub}[1]{\ensuremath{\bar{#1}}\xspace}
\newcommand{\lb}[1]{\ensuremath{\ubar{#1}}\xspace}

\newcommand{\powerset}{\ensuremath{\mathcal{P}}\xspace}
% set of halfspaces representing the faces of some polytope (compressor config polytope, tv bound polytope, etc.)
\newcommand{\setFacets}[1]{\ensuremath{\mathcal{H}_{#1}}\xspace}

%%----------------------------------------------------------
%% all used mathcal letters
%%----------------------------------------------------------
% A - arcs
% C - compressor configurations
% F - flow directions
% G - fence groups
% H - configuration facets(hyperplanes)
% M - machines (maybe unify with U?)
% O - operation modes
% P - power set
% Q - valid operation mode/flowdirection combinations
% S - Simple states
% T - time steps
% U - units (maybe unify with M?)
% V - vertices
% W - flow direction conditions

%%-----------------------------------------------------------
%% Graph
%%----------------------------------------------------------
\newcommand{\graph}{\ensuremath{G}\xspace}
\newcommand{\generalGraph}{\ensuremath{\graph=(\setVertices,\setArcs)}\xspace}
\newcommand{\netmodelGraph}{\ensuremath{\graph=(\setVertices,\setPipes \cup \setRegulators \cup \setValves \cup \setArtificialLinks)}\xspace}

% nodes
\newcommand{\setVertices}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\setVerticesAll}{\ensuremath{\setVertices = \setBoundaryNodes \cup \setInnerNodes}\xspace}
\newcommand{\setEntries}{\ensuremath{\setVertices^{+}}\xspace}
\newcommand{\setExits}{\ensuremath{\setVertices^{-}}\xspace}
\newcommand{\setBoundaryNodes}{\ensuremath{\setVertices^\mathrm{b}}\xspace}
\newcommand{\setBoundaryNodesAll}{\ensuremath{\setEntries \cup \setExits}\xspace}
\newcommand{\setInnerNodes}{\ensuremath{\setVertices^{0}}\xspace}
\newcommand{\setFenceNodes}{\ensuremath{\setVertices^{\mathrm{fn}}}\xspace}
\newcommand{\setFenceNodesNaviStation}[1]{\ensuremath{\setFenceNodes_{i}}\xspace}
\newcommand{\setArtificialNodes}{\ensuremath{\setVertices^{\mathrm{ar}}}\xspace}
\newcommand{\setArtificialNodesNaviStation}[1]{\ensuremath{\setArtificialNodes_{#1}}\xspace}

% arcs
\newcommand{\setArcs}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\setArcsAllStationModel}{\ensuremath{\setArcs = \setPipes \cup \setValves \cup \setResistors \cup \setRegulators \cup \setCompressorStations}\xspace}
\newcommand{\setPipes}{\ensuremath{\setArcs^{\mathrm{pi}}}\xspace}
\newcommand{\setRegulators}{\ensuremath{\setArcs^{\mathrm{rg}}}\xspace}
\newcommand{\setValves}{\ensuremath{\setArcs^{\mathrm{va}}}\xspace}
\newcommand{\setValvesNS}{\ensuremath{\setArcs^{\mathrm{va-s}}}\xspace}
\newcommand{\setResistors}{\ensuremath{\setArcs^{\mathrm{rs}}}\xspace}
\newcommand{\setCompressorStations}{\ensuremath{\setArcs^{\mathrm{cs}}}\xspace}

% station model specific arcs
\newcommand{\setRegulatorsControllable}{\ensuremath{\setArcs^{\mathrm{rg-c}}}\xspace}
\newcommand{\setRegulatorsNonControllable}{\ensuremath{\setArcs^{\mathrm{rg-nc}}}\xspace}
\newcommand{\setRegulatorsNonControllableActive}{\ensuremath{\setArcs^{\mathrm{rg-nca}}}\xspace}
\newcommand{\setRegulatorsNonControllableFixed}{\ensuremath{\setArcs^{\mathrm{rg-ncf}}}\xspace}
\newcommand{\setRegulatorsNonControllableAll}{\ensuremath{\setRegulatorsNonControllable := \setRegulatorsNonControllableActive\cup\setRegulatorsNonControllableFixed}\xspace}

% special compressor station sets
\newcommand{\setCompressorUnits}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\setCompressorUnitsI}[1]{\ensuremath{\setCompressorUnits_{#1}}\xspace}
\newcommand{\setCompressorConfigurations}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setCompressorConfigurationsUsingUnit}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setConfigurationFacets}[1]{\ensuremath{\setFacets{#1}}\xspace}

% navi station specific (net model)
\newcommand{\naviStationGraph}[1]{\ensuremath{G}_{#1}\xspace}
\newcommand{\naviStationGraphAll}[1]{\ensuremath{\naviStationGraph{#1}=(\setVerticesNaviStation{#1},\setArtificialLinksNaviStation{#1})\xspace}}
\newcommand{\setVerticesNaviStation}[1]{\ensuremath{\setVertices}_{#1}\xspace}
\newcommand{\setArtificialLinksNaviStation}[1]{\ensuremath{\setArcs^{\mathrm{ar}}}_{#1}\xspace}
\newcommand{\nNaviStations}{\ensuremath{m}\xspace}

% navi station specific (station model)
\newcommand{\setNSModes}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\setNSValidPairs}{\ensuremath{\mathcal{Q}}\xspace} % valid pairs of operation modes and flow directions
\newcommand{\setNSFenceGroups}{\ensuremath{\mathcal{G}}\xspace}
% old commands, deprecated, just used to create the latexdiff for the stationModelPaper
\newcommand{\setOldNSValidPairs}{\ensuremath{\mathcal{OF}}\xspace}
\newcommand{\setOldNSFenceGroups}{\ensuremath{\mathcal{FG}}\xspace}
% end of old commands
\newcommand{\setBoundaryNodesExitP}{\ensuremath{\setVertices^\mathrm{b-ex}}\xspace}

%%-----------------------------------------------------------
%% Time
%%----------------------------------------------------------
\newcommand{\setTimesteps}{\ensuremath{\mathcal{T}_0}\xspace}
\newcommand{\setTimestepsNoZero}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\nTimesteps}{\ensuremath{k}\xspace}
\newcommand{\setTimestepsAll}{\ensuremath{\setTimesteps := \{0, \dots, \nTimesteps\}}\xspace}
\newcommand{\setTimestepsNoZeroAll}{\ensuremath{\setTimestepsNoZero := \setTimesteps\setminus\{0\}}\xspace}
\newcommand{\granularity}{\ensuremath{\tau}\xspace}
\newcommand{\granularityI}[1]{\ensuremath{\granularity(#1)}\xspace}

%%-----------------------------------------------------------
%% Supplies and demands
%%----------------------------------------------------------
\newcommand{\inflow}{\ensuremath{d}}
\newcommand{\paramInflowValue}[2]{\ensuremath{D_{#1,#2}}\xspace}
\newcommand{\paramSupplyValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramDemandValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramSupplyUB}[2]{\ensuremath{\ub{D}_{#1,#2}}\xspace}
\newcommand{\paramDemandUB}[2]{\ensuremath{\lb{D}_{#1,#2}}\xspace}
\newcommand{\inflowI}[1]{\ensuremath{\inflow_{#1}}\xspace}
\newcommand{\paramInflowValueUB}[2]{\ensuremath{\ub{\inflow}_{#1,#2}}\xspace}
\newcommand{\paramInflowValueLB}[2]{\ensuremath{\lb{\inflow}_{#1,#2}}\xspace}
\newcommand{\varSupplyValue}[2]{\ensuremath{\varInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \varInflowValue
\newcommand{\varDemandValue}[2]{\ensuremath{\varInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \varInflowValue

% station model demands for inflow and pressure
\newcommand{\demandPressure}[1]{\ensuremath{\hat{\press}_{#1}}\xspace}
\newcommand{\demandInflow}[1]{\ensuremath{\hat{\inflow}_{#1}}\xspace}

%%-----------------------------------------------------------
%% Pressure
%%----------------------------------------------------------
\newcommand{\press}{\ensuremath{p}\xspace}
\newcommand{\pressI}[1]{\ensuremath{\press_{#1}}\xspace}
\newcommand{\pressUB}[1]{\ensuremath{\ub{\press}_{#1}}\xspace}
\newcommand{\pressLB}[1]{\ensuremath{\lb{\press}_{#1}}\xspace}
\newcommand{\inflowPressUB}[1]{\ensuremath{\paramPressUB{#1}^{\mathrm{act}}}\xspace} % act => active
\newcommand{\inflowPressLB}[1]{\ensuremath{\paramPressLB{#1}^{\mathrm{act}}}\xspace} % act => active

%%-----------------------------------------------------------
%% Flow
%%----------------------------------------------------------
\newcommand{\mFlow}{\ensuremath{q}\xspace}
\newcommand{\mFlowI}[1]{\ensuremath{\mFlow_{#1}}\xspace}
\newcommand{\mFlowFwd}[1]{\ensuremath{\mFlow{#1}^{\rightarrow}}\xspace}
\newcommand{\mFlowBwd}[1]{\ensuremath{\mFlow{#1}^{\leftarrow}}\xspace}
\newcommand{\mFlowUB}[1]{\ensuremath{\ub{\mFlow}_{#1}}\xspace}
\newcommand{\mFlowLB}[1]{\ensuremath{\lb{\mFlow}_{#1}}\xspace}
\newcommand{\fenceFlow}[1]{\ensuremath{\varArcFlow{#1}^\mathrm{fn}}\xspace}

%%-----------------------------------------------------------
%% Netmodel Navi Station
%%----------------------------------------------------------
\newcommand{\setArtificialLinks}{\ensuremath{\setArcs^{\mathrm{ar}}}\xspace}
\newcommand{\setShortcuts}{\ensuremath{\setArcs^{\mathrm{ar-sc-bi}}}\xspace}
\newcommand{\setShortcutsNaviStation}[1]{\ensuremath{\setShortcuts_{#1}}\xspace}
\newcommand{\setRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{ar-rg}}}\xspace}
\newcommand{\setRegulatorArcsNaviStation}[1]{\ensuremath{\setRegulatorArcs_{#1}}\xspace}
\newcommand{\setCompressorArcs}{\ensuremath{\setArcs^{\mathrm{ar-cp}}}\xspace}
\newcommand{\setCompressorArcsNaviStation}[1]{\ensuremath{\setCompressorArcs_{#1}}\xspace}
\newcommand{\setCombinedArcs}{\ensuremath{\setArcs^{\mathrm{ar-cb}}}\xspace}
\newcommand{\setCombinedArcsNaviStation}[1]{\ensuremath{\setCombinedArcs_{#1}}\xspace}

\newcommand{\setBiRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{ar-rg-bi}}}\xspace}
\newcommand{\setBiRegulatorArcsNaviStation}[1]{\ensuremath{\setBiRegulatorArcs_{#1}}\xspace}
\newcommand{\setBiCompressorArcs}{\ensuremath{\setArcs^{\mathrm{ar-cp-bi}}}\xspace}
\newcommand{\setBiCompressorArcsNaviStation}[1]{\ensuremath{\setBiCompressorArcs_{#1}}\xspace}
\newcommand{\setBiCombinedArcs}{\ensuremath{\setArcs^{\mathrm{ar-cb-bi}}}\xspace}
\newcommand{\setBiCombinedArcsNaviStation}[1]{\ensuremath{\setBiCombinedArcs_{#1}}\xspace}

\newcommand{\setDirectedArcs}{\ensuremath{\setArcs^{\mathrm{ar-di}}}\xspace}
\newcommand{\setDirectedArcsNaviStation}[1]{\ensuremath{\setDirectedArcs_{#1}}\xspace}
\newcommand{\setBiArcs}{\ensuremath{\setArcs^{\mathrm{ar-bi}}}\xspace}
\newcommand{\setBiArcsNaviStation}[1]{\ensuremath{\setBiArcs_{#1}}\xspace}
\newcommand{\setCompressingArcs}{\ensuremath{\setArcs^{\mathrm{ar-co}}}\xspace}
\newcommand{\setCompressingArcsNaviStation}[1]{\ensuremath{\setCompressingArcs_{#1}}\xspace}

\newcommand{\setSimpleStates}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\setSimpleStatesNaviStation}[1]{\ensuremath{\mathcal{S}_{#1}}\xspace}
\newcommand{\simpleState}{\ensuremath{s}\xspace}
\newcommand{\simpleStateFlowDirections}{\ensuremath{\simpleState^{\flowDirection}}\xspace}
\newcommand{\simpleStateLinksMandatoryActive}{\ensuremath{\simpleState^{on}}\xspace}
\newcommand{\simpleStateLinksMandatoryInactive}{\ensuremath{\simpleState^{off}}\xspace}

\newcommand{\varActivation}[2]{\ensuremath{x_{#1,#2}}\xspace}
\newcommand{\varFlowDirectionActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varSimpleStateActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkActivationFwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\rightarrow}}\xspace}
\newcommand{\varArtificialLinkActivationBwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\leftarrow}}\xspace}
\newcommand{\varCombinedLinkRegulatingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{rg}}}\xspace}
\newcommand{\varCombinedLinkCompressingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{cp}}}\xspace}

\newcommand{\varChange}[2]{\ensuremath{\delta_{#1,#2}}\xspace}
\newcommand{\varFlowDirectionChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varSimpleStateChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkChangeOn}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{on}}}\xspace}
\newcommand{\varArtificialLinkChangeOff}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{off}}}\xspace}

\newcommand{\setFlowDirectionConditions}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\setFlowDirectionConditionsNaviStation}[1]{\ensuremath{\setFlowDirectionConditions_{i}}\xspace}

%%-----------------------------------------------------------
%% Machines, Power, Compression Ratio, and Betriebsvolumenstrom
%%-----------------------------------------------------------
\newcommand{\setMachinesNaviStation}[1]{\ensuremath{\mathcal{M}}_{#1}\xspace}
\newcommand{\setMachinesNaviStationOnLink}[2]{\ensuremath{\setMachinesNaviStation{#1}^{#2}}\xspace}
\newcommand{\generalMachine}{\ensuremath{m}\xspace}
\newcommand{\machine}[1]{\ensuremath{\generalMachine_{#1}}\xspace}

\newcommand{\varAssignMachineToLink}[3]{\ensuremath{y_{#1,#2,#3}}\xspace}

\newcommand{\paramMaxNumberMachinesLink}{\ensuremath{M_a^{\mathrm{max}}}\xspace}
\newcommand{\paramMaxCompressionRatio}[2]{\ensuremath{R_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxPower}[2]{\ensuremath{\power_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxBetriebsVolumenstrom}[2]{\ensuremath{\volumetricFlow_{\machine{#1},#2}}\xspace}

\newcommand{\varCompressionRatio}[2]{\ensuremath{r_{#1,#2}}\xspace}
\newcommand{\varPower}[2]{\ensuremath{\pi_{#1,#2}}\xspace}
\newcommand{\varBetriebsVolumenstrom}[2]{\ensuremath{\omega_{#1,#2}}\xspace}
\newcommand{\varMaxPower}[2]{\ensuremath{\varPower{#1}{#2}^{max}}\xspace}
\newcommand{\varMaxBetriebsVolumenstrom}[2]{\ensuremath{\varBetriebsVolumenstrom{#1}{#2}^{max}}\xspace}

\newcommand{\paramMaxCompressionRatioLink}[2]{\ensuremath{\ub{R}_{#1,#2}}\xspace}
\newcommand{\paramPressureUBCompression}[2]{\ensuremath{\paramPressureUB{#1}{#2}^{\mathrm{out}}}\xspace}


%%-----------------------------------------------------------
%% Smoothing
%%-----------------------------------------------------------

\newcommand{\generalSmoothing}{\ensuremath{\delta}\xspace}
\newcommand{\varSmoothingPressurePos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press+}}\xspace}
\newcommand{\varSmoothingPressureNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press-}}\xspace}
\newcommand{\varSmoothingInflowPos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow+}}\xspace}
\newcommand{\varSmoothingInflowNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow-}}\xspace}

%%-----------------------------------------------------------
%% Flow Direction (used in both models)
%%-----------------------------------------------------------
\newcommand{\setFlowDirectionsNavi}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\setFlowDirectionsNaviStation}[1]{\ensuremath{\setFlowDirectionsNavi_{#1}}\xspace}
\newcommand{\flowDirection}{\ensuremath{f}\xspace}
\newcommand{\flowDirectionEntries}{\ensuremath{\flowDirection^{+}}\xspace}
\newcommand{\flowDirectionExits}{\ensuremath{\flowDirection^{-}}\xspace}
\newcommand{\pressUBExitFG}[1]{\ensuremath{\ub{\press}_{#1}^{\mathrm{exit}}}\xspace}

%%-----------------------------------------------------------
%% Mode variables
%%----------------------------------------------------------
\newcommand{\mode}{\ensuremath{m}\xspace}
\newcommand{\modeOp}[1]{\ensuremath{\mode_{#1}^\mathrm{op}}\xspace}
\newcommand{\modeCl}[1]{\ensuremath{\mode_{#1}^\mathrm{cl}}\xspace}
\newcommand{\modeBy}[1]{\ensuremath{\mode_{#1}^\mathrm{by}}\xspace}
\newcommand{\modeAc}[1]{\ensuremath{\mode_{#1}^\mathrm{ac}}\xspace}
\newcommand{\modeCv}[1]{\ensuremath{\mode_{#1}^\mathrm{cvcl}}\xspace} % closed because of a check valve
\newcommand{\modeFix}[1]{\ensuremath{\mode_{#1}^\mathrm{fix}}\xspace} % fixed mode for non-controllable regulators
\newcommand{\modeX}[1]{\ensuremath{\mode_{#1}^\mathrm{x}}\xspace}
\newcommand{\cfg}[1]{\ensuremath{\mode_{#1}^\mathrm{cf}}\xspace}
\newcommand{\opMode}[1]{\ensuremath{\mode_{#1}^\mathrm{om}}\xspace}
\newcommand{\flowDir}[1]{\ensuremath{\mode_{#1}^\mathrm{fd}}\xspace}


%%-----------------------------------------------------------
%% Mode specific pressure and flow variables
%%----------------------------------------------------------
\newcommand{\pressBy}[1]{\ensuremath{\pressI{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowBy}[1]{\ensuremath{\mFlowI{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfg}[1]{\ensuremath{\mFlowI{#1}^\mathrm{cf}}\xspace}
%% upper bounds for all of them
\newcommand{\pressByUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{cf}}\xspace}
%% lower bounds for all of them
\newcommand{\pressByLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{cf}}\xspace}

%%-----------------------------------------------------------
%% Slack variables
%%----------------------------------------------------------
\newcommand{\slack}{\ensuremath{\sigma}\xspace}
\newcommand{\slackPPos}[1]{\ensuremath{\slack_{#1}^{\press+}}\xspace}
\newcommand{\slackPNeg}[1]{\ensuremath{\slack_{#1}^{\press-}}\xspace}
\newcommand{\slackQPos}[1]{\ensuremath{\slack_{#1}^{\inflow+}}\xspace}
\newcommand{\slackQNeg}[1]{\ensuremath{\slack_{#1}^{\inflow-}}\xspace}

%%-----------------------------------------------------------
%% Target values
%%----------------------------------------------------------
%% target value types
\newcommand{\PIN}{\pressI{\ell}\xspace}
\newcommand{\POUT}{\pressI{r}\xspace}
\newcommand{\MINPIN}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MAXPIN}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MINPOUT}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MAXPOUT}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MINQ}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\MAXQ}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\SETQ}{\ensuremath{\mFlowI{\mathrm{set}}}\xspace}

%% sets
\newcommand{\setTargetValues}{\ensuremath{\Gamma}\xspace} % all TVs
\newcommand{\setTargetValuesI}[1]{\ensuremath{\setTargetValues_{#1}}\xspace} % ... of some element
\newcommand{\setStaPush}{\ensuremath{\Theta}\xspace} % all stable/pushing TV combinations
\newcommand{\setStaPushI}[1]{\ensuremath{\setStaPush_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushActive}{\ensuremath{\setStaPush^\mathrm{ac}}\xspace} % all combinations for active mode
\newcommand{\setStaPushActiveI}[1]{\ensuremath{\setStaPushActive_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushOpen}{\ensuremath{\setStaPush^\mathrm{op}}\xspace} % all combinations for open mode
\newcommand{\setStaPushOpenI}[1]{\ensuremath{\setStaPushOpen_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushClosed}{\ensuremath{\setStaPush^\mathrm{cl}}\xspace} % all combinations for closed mode
\newcommand{\setStaPushClosedI}[1]{\ensuremath{\setStaPushClosed_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushXI}[1]{\ensuremath{\setStaPush^\mathrm{x}_{#1}}\xspace} % all combination for x mode for some element
\newcommand{\setTVBPolysI}[1]{\ensuremath{\Phi_{#1}}\xspace}
\newcommand{\setTVBPolysActiveI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac}}\xspace}
\newcommand{\setTVBPolysBypassI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{by}}\xspace}
\newcommand{\setTVBPolysClosedI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{cl}}\xspace}
\newcommand{\setTVBPolysActiveQI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}Q}}\xspace}
\newcommand{\setTVBPolysActivePInI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}p_{in}}}\xspace}
\newcommand{\setTVBPolysActivePOutI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}p_{out}}}\xspace}
\newcommand{\setTVBPolysActiveXI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}X}}\xspace}
\newcommand{\setTVBPolysXI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{X}}\xspace}
\newcommand{\setTVQuantities}{\ensuremath{\Omega}\xspace}

%% vars
\newcommand{\tv}{\ensuremath{\tau}\xspace}
\newcommand{\tvI}[1]{\ensuremath{\tv_{#1}}\xspace}
\newcommand{\lbTVI}[1]{\ensuremath{\lb{\tv}_{#1}}\xspace}
\newcommand{\ubTVI}[1]{\ensuremath{\ub{\tv}_{#1}}\xspace}

% set values

\newcommand{\tvSet}{\ensuremath{\tv^\mathrm{set}}\xspace}
\newcommand{\tvSetI}[1]{\ensuremath{\tvSet_{#1}}\xspace}

% target value bound polytope variable
\newcommand{\tvPolyI}[1]{\ensuremath{\phi_{#1}}\xspace}

% target value stable pushing combination variable
\newcommand{\tvCombi}{\ensuremath{\theta}\xspace}
\newcommand{\tvCombiI}[1]{\ensuremath{\tvCombi_{#1}}\xspace}
\newcommand{\funcTvPrio}{\ensuremath{\varphi}\xspace} % target value priority function
\newcommand{\funcTvPrioI}[1]{\ensuremath{\funcTvPrio(#1)}\xspace} % .. with argument


%%-----------------------------------------------------------
%% Objective change variables
%%----------------------------------------------------------
\newcommand{\objVar}{\ensuremath{\delta}\xspace}
\newcommand{\objVarI}[1]{\ensuremath{\delta_{#1}}\xspace}
\newcommand{\opModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{om}}}\xspace}
\newcommand{\unitStart}[1]{\ensuremath{\objVarI{#1}^{\mathrm{us}}}\xspace}
\newcommand{\regModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg}}}\xspace}
\newcommand{\xPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-pl}}}\xspace}
\newcommand{\xPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-pr}}}\xspace}
\newcommand{\xQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-q}}}\xspace}
\newcommand{\rgPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-pl}}}\xspace}
\newcommand{\rgPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-pr}}}\xspace}
\newcommand{\rgQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-q}}}\xspace}
\newcommand{\csPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-pl}}}\xspace}
\newcommand{\csPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-pr}}}\xspace}
\newcommand{\csQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-q}}}\xspace}
\newcommand{\tvChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{tv}}}\xspace}
\newcommand{\tvSetChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{set}}}\xspace}

%%-----------------------------------------------------------
%% Objective cost parameters
%%-----------------------------------------------------------
\newcommand{\cost}{\ensuremath{w}\xspace}
\newcommand{\costSlackP}{\ensuremath{\cost^{\slack\mathrm{-p}}}\xspace}
\newcommand{\costSlackQ}{\ensuremath{\cost^{\slack\mathrm{-d}}}\xspace}
\newcommand{\costOpModes}{\ensuremath{\cost^\mathrm{om}}\xspace}
\newcommand{\costUnitStarts}{\ensuremath{\cost^\mathrm{us}}\xspace}
\newcommand{\costRgModeChg}{\ensuremath{\cost^\mathrm{rg}}\xspace}
\newcommand{\costXPLChg}{\ensuremath{\cost^\mathrm{X-pl}}\xspace}
\newcommand{\costXPRChg}{\ensuremath{\cost^\mathrm{X-pr}}\xspace}
\newcommand{\costXQChg}{\ensuremath{\cost^\mathrm{X-q}}\xspace}
\newcommand{\costRgPLChg}{\ensuremath{\cost^\mathrm{rg-pl}}\xspace}
\newcommand{\costRgPRChg}{\ensuremath{\cost^\mathrm{rg-pr}}\xspace}
\newcommand{\costRgQChg}{\ensuremath{\cost^\mathrm{rg-q}}\xspace}
\newcommand{\costCsPLChg}{\ensuremath{\cost^\mathrm{cs-pl}}\xspace}
\newcommand{\costCsPRChg}{\ensuremath{\cost^\mathrm{cs-pr}}\xspace}
\newcommand{\costCsQChg}{\ensuremath{\cost^\mathrm{cs-q}}\xspace}
\newcommand{\costFlowDirectionChange}{\ensuremath{\cost^f}\xspace}
\newcommand{\costFlowDirectionChangeNaviStation}[1]{\ensuremath{\costFlowDirectionChange_{#1}}\xspace}
\newcommand{\costOriginalSimpleStateChange}{\ensuremath{\tilde{\cost}^s}\xspace}
\newcommand{\costSimpleStateChange}{\ensuremath{\cost^s}\xspace}
\newcommand{\costArtificialLinkChange}{\ensuremath{\cost^a}\xspace}
\newcommand{\costCompressingLinkOn}[1]{\ensuremath{\cost_{#1}^{\mathrm{cp-act}}}\xspace}
\newcommand{\costCompressingLinkValue}[1]{\ensuremath{\cost_{#1}^{\mathrm{cp-val}}}\xspace}
\newcommand{\costSmoothingPressure}{\ensuremath{\cost^{\mathrm{sm-p}}}\xspace}
\newcommand{\costSmoothingFlow}{\ensuremath{\cost^{\mathrm{sm-q}}}\xspace}
\newcommand{\costTVChg}{\ensuremath{\cost^\mathrm{tv}}\xspace}

%%-----------------------------------------------------------
%% Other physical quantities
%%----------------------------------------------------------
\newcommand{\velo}{\ensuremath{v}\xspace}
\newcommand{\absVelo}[1]{\ensuremath{|\velo_{#1}|}\xspace}
\newcommand{\gasConst}{\ensuremath{R}\xspace}
\newcommand{\sGasConst}{\ensuremath{\gasConst_{\mathrm{s}}}\xspace}
\newcommand{\temp}{\ensuremath{T}\xspace}
\newcommand{\tempI}[1]{\ensuremath{\temp{#1}}\xspace}
\newcommand{\zFact}{\ensuremath{z}\xspace}
\newcommand{\zFactI}[1]{\ensuremath{\zFact_{#1}}\xspace}
\newcommand{\vol}{\ensuremath{V}\xspace}
\newcommand{\amountOfSubstance}{\ensuremath{n}\xspace}
\newcommand{\pseudoP}{\ensuremath{\press^\mathrm{c}}\xspace}
\newcommand{\pseudoT}{\ensuremath{\temp^\mathrm{c}}\xspace}
\newcommand{\molMass}{\ensuremath{M}\xspace}
\newcommand{\len}{\ensuremath{L}\xspace}
\newcommand{\lenI}[1]{\ensuremath{\len_{#1}}\xspace}
\newcommand{\area}{\ensuremath{A}\xspace}
\newcommand{\areaI}[1]{\ensuremath{\area_{#1}}\xspace}
\newcommand{\diam}{\ensuremath{D}\xspace}
\newcommand{\diamI}[1]{\ensuremath{\diam_{#1}}\xspace}
\newcommand{\slope}{\ensuremath{s}\xspace}
\newcommand{\slopeI}[1]{\ensuremath{\slope_{#1}}\xspace}
\newcommand{\fric}{\ensuremath{\lambda}\xspace}
\newcommand{\fricI}[1]{\ensuremath{\fric_{#1}}\xspace}
\newcommand{\rough}{\ensuremath{k}\xspace}
\newcommand{\roughI}[1]{\ensuremath{\rough_{#1}}\xspace}
\newcommand{\dynVisc}{\ensuremath{\eta}\xspace}
\newcommand{\gravAcc}{\ensuremath{g}\xspace}
\newcommand{\dens}{\ensuremath{\rho}\xspace}
\newcommand{\nDens}{\ensuremath{\dens_0}\xspace} % subscript is used in the code for this and should be left free, if possible
\newcommand{\vFlow}{\ensuremath{Q}\xspace}
\newcommand{\nvFlow}{\ensuremath{Q^0}\xspace}
\newcommand{\nvFlowI}[1]{\ensuremath{Q^0_{#1}}\xspace}
\newcommand{\timeDiff}{\ensuremath{\Delta_t}\xspace} %equals \tau(t) - \tau(t-1)
\newcommand{\power}{\ensuremath{P}\xspace}
\newcommand{\adEnth}{\ensuremath{H_\mathrm{ad}}\xspace}
\newcommand{\adEff}{\ensuremath{\eta_\mathrm{ad}}\xspace} % \eta is already the dyn viscosity, but it's the same in the gas book
\newcommand{\isenExp}{\ensuremath{\kappa}\xspace}

%%-----------------------------------------------------------
%% Other element parameters
%%----------------------------------------------------------
\newcommand{\height}[1]{\ensuremath{h_{#1}}\xspace}
\newcommand{\drag}[1]{\ensuremath{\zeta_{#1}}\xspace}
\newcommand{\machinePDiffUB}{\ensuremath{\ub{\Delta}_\press}\xspace}

%%-----------------------------------------------------------
%% Number sets
%%----------------------------------------------------------
\newcommand{\setReals}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\setRealsNonNeg}{\ensuremath{\setReals_{\geq 0}}\xspace}
\newcommand{\setRealsNonPos}{\ensuremath{\setReals_{\leq 0}}\xspace}
\newcommand{\setRealsNeg}{\ensuremath{\setReals_{< 0}}\xspace}
\newcommand{\setRealsPos}{\ensuremath{\setReals_{> 0}}\xspace}
\newcommand{\setNaturalNumbers}{\ensuremath{\mathbb{N}}\xspace}
